OntoMerger: An Ontology Integration Library for Deduplicating and Connecting Knowledge Graph Nodes

Duplication of nodes is a common problem encountered when building knowledge graphs (KGs) from heterogeneous datasets, where it is crucial to be able to merge nodes having the same meaning. OntoMerger is a Python ontology integration library whose functionality is to deduplicate KG nodes. Our approach takes a set of KG nodes, mappings and disconnected hierarchies and generates a set of merged nodes together with a connected hierarchy. In addition, the library provides analytic and data testing functionalities that can be used to fine-tune the inputs, further reducing duplication, and to increase connectivity of the output graph. OntoMerger can be applied to a wide variety of ontologies and KGs. In this paper we introduce OntoMerger and illustrate its functionality on a real-world biomedical KG.

==> algorithms/batching_algorithm.tex <==
	\begin{algorithm}[h!]
{\small		\DontPrintSemicolon
		\SetAlgoLined
		\KwData{$\mathcal{B}$ -- Batch of (drug A, drug B, cell line, label) tuples.\\
		$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\mathcal{G}$ -- Graph of interest.\\
		$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,s$ -- Sample size for multi-scale approximation.\\
		}
		\KwResult{$\mathcal{L}$ -- Average loss on batch $\mathcal{B}$.}
$\mathcal{L}\leftarrow 0 $\;
\For{$(d,d',c,y) \in \mathcal{B}$}{
$\overline{\textbf{m}}_{d}\leftarrow \textbf{Sample Representation}(\mathcal{G},d,s)$\;
$\overline{\textbf{m}}_{d'}\leftarrow \textbf{Sample Representation}(\mathcal{G},d',s)$\;
$\textbf{h}_{(d,d',c)}\leftarrow [\overline{\textbf{m}}_{d} \| \overline{\textbf{m}}_{d'} \|  \textbf{h}_{c}]$\;
$\hat{y}_{(d,d',c)} \leftarrow  f_{\Theta_H}(\textbf{h}_{(d,d',c)})$\;

$\mathcal{L} \leftarrow  \mathcal{L} + \ell(y; \hat{y}_{(d,d',c)})/|\mathcal{B}|$\;
}
}
		\caption{Mini-batch based forward pass of MOOMIN-A with approximate multi-scale multimodal representations.}\label{alg:batching}
	\end{algorithm}
\vspace{-5mm}



==> algorithms/sampling_algorithm.tex <==
	\begin{algorithm}[h!]
{\small		\DontPrintSemicolon
		\SetAlgoLined
		\KwData{$\mathcal{G}$ -- Bipartite drug -- protein interaction graph.\\
		$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,d$ -- Source drug of interest.\\
		$\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,s$ -- Sample size.\\
		}
		\KwResult{$\overline{\textbf{m}}_d$ -- Sampled multi-scale representation of drug $\textit{d}.$}
$\widetilde{\textbf{m}}^0_d\leftarrow f_{\Theta_{D}}(\mathcal{M}_d)$\;
$\overline{\textbf{m}}_d\leftarrow\textbf{0}$\;
\For{$i \in \left \{1,\dots ,s\right \}$}{
$\widetilde{d}\leftarrow d$\;
$\widetilde{\textbf{m}}_d\leftarrow\widetilde{\textbf{m}}^0_d$\;
    \For{$l \in \left \{1,\dots ,r\right \}$}{
            \uIf{$l \mod 2 = 1$}{
            $\widetilde{p} \leftarrow \textbf{Random neighbor}(\mathcal{G}, \widetilde{d})$\;
            $\widetilde{\textbf{m}}^l_d \leftarrow f_{\Theta_p} (\textbf{x}_{\widetilde{p}}) $\;
            $\widetilde{\textbf{m}}_d \leftarrow [\widetilde{\textbf{m}}_d   \|  \widetilde{\textbf{m}}^l_d]$\;
            }
            \Else{
            $\widetilde{d} \leftarrow \textbf{Random neighbor}(\mathcal{G}, \widetilde{p})$\;
            $\widetilde{\textbf{m}}^l_{\widetilde{d}} \leftarrow f_{\Theta_D} (\mathcal{M}_d) $\;
            $\widetilde{\textbf{m}}_d \leftarrow [\widetilde{\textbf{m}}_d   \|  \widetilde{\textbf{m}}^l_d  ]$\;
            }
            }
            $\overline{\textbf{m}}_d \leftarrow \overline{\textbf{m}}_d + \widetilde{\textbf{m}}_d$ \;
}
            $\overline{\textbf{m}}_d \leftarrow \overline{\textbf{m}}_d /s$\;
}
		\caption{Approximate truncated random walk sampled multi-scale drug representation forward pass with MOOMIN.}\label{alg:sampling_algorithm}
	\end{algorithm}
	



==> original/0.abstract-bak.tex <==
\begin{abstract}
Duplication of nodes is a common problem encountered when building knowledge graphs. It is crucial to be able to merge nodes having the same meaning. OntoMerger is a Python ontology integration library that provides functionality to deduplicate knowledge graph nodes. Our approach inputs knowledge graph nodes, mappings and disconnected hierarchies and outputs merged nodes together with a connected hierarchy. In addition, the library provides analytics and data testing functionalities that can be used to fine-tune the inputs, further reduce duplication and to increase connectivity of the output graph. OntoMerger can be applied to a wide variety of ontologies. We showcase its main functionality on a real-world biomedical knowledge graph.
\end{abstract}

==> original/1.introduction-bak.tex <==
\section{Introduction}
Complex knowledge graphs (KGs) (\cite{geleta2021biological}, \cite{sinha2015overview}) are often built from multiple overlapping but heterogeneous data sets. For example, a biomedical KG can include separate data sets providing information about genes, diseases, compounds and relations between these entities. Typically source data sets rely on diverse ontologies to refer to the same concepts with no obvious mapping between the ontologies. In addition data version discrepancy can lead to duplication when concepts get deprecated and identifiers reassigned. On a large scale these issues cause syntactic and semantic heterogeneity in the resulting graph. Heterogeneity in turn leads to fragmented knowledge and negatively impacts downstream machine learning applications. 

By organising concepts of the same domain into a hierarchy we can improve accuracy of machine learning models, such as pattern recognition (ref?). Hierarchies facilitate finding similar concepts based on neighbourhoods. However, hierarchies %of different ontologies 
may be incompatible, and a simple merge could lead to inconsistencies. % (loops etc.).

OntoMerger tackles these challenges by using a scaffolding ontology together with  mappings and concept hierarchies to produce an integrated domain ontology with a single DAG hierarchy. By design this ontology does not necessarily retain complete knowledge for all the integrated concepts, such as hierarchical connections and the granularity of the original conceptualisation.  
OntoMerger relies on mappings provided by the users and produces inferred ones.  
The library is open source\footnote{https://github.com/AstraZeneca/onto\_merger}, implemented in Python~\cite{vanrossum1995python}, and it is available to download\footnote{https://pypi.org/project/onto\_merger} as a package via PyPi~\cite{pypi}.  
The library processes data in a tabular format using the Pandas~\cite{mckinney2011pandas} package.  
For producing the hierarchy, OntoMerger converts hierarchy triples into graph objects 
and runs queries for finding paths (using NetworKit~\cite{staudt2016networkit}), as well as for counting 
sub-graphs (using NetworkX~\cite{hagberg2008exploring}).  
To ensure stable performance, input and output data is tested using the 
Great Expectations~\cite{greatexpectations} validation framework.  
In addition, the library provides in-depth analysis by profiling all consumed and produced 
data using the Pandas Profiling~\cite{pandasprofiling} package.  
Insights about the input, intermediate, and produced data (i.e. the domain ontology), results of data profiling and data validation, 
and metrics about the inner workings of the library are presented in an HTML report, shown in Figure \ref{fig:report}.

==> original/2.related_work-bak.tex <==
\section{Related work}\label{sec:related_work}

The ontology integration challenge has been in the focus of the research community for a long time~\cite{osman2021survey}. While the \emph{ontology matching} problem of automated generation of mappings between ontologies has attracted the most attention~\cite{euzenat2007ontology}, using these mappings to produce a coherent, integrated ontology often presented a non-trivial task due to the need to satisfy the merge requirements~\cite{pottinger2003merging}, such as preserving correctness and coherence, maintaining acyclicity, and prohibition of redundancy. To satisfy these requirements existing algorithms often try to modify the alignments~\cite{stoilos2018novel,Solimando2017,udrea2007iliads} or even to repair the  ontologies themselves~\cite{jimenez-ruiz2009integration,raunich2014atom,fahad2012dkpaom}. 

Despite the significant effort invested into solving the ontology integration problem over the years, existing methods do not always satisfy the requirements of practical use cases in the context of large scale data science scenarios, which makes them hard to apply. For example, existing systems usually rely on OWL semantics and explicit constraints defined in source ontologies. However, there might also exist implicit ones: e.g., even if two concepts in the same ontology might not be declared as disjoint, we may not want them to be merged into one as a result of ontology integration. Also, most of existing RDF/OWL tools are implemented in Java, while nowadays many data science practitioners having to deal with ontology integration prefer the Python ecosystem.

==> tables/input_output_comparison.tex <==
\begin{table}[!ht]
% \label{eval:input_output_comparison}
\centering
\scalebox{0.80}{
\begin{tabular}{|l|r|r|}
\hline
    \textbf{Metric} & \textbf{Count (Input)} & \textbf{Count (Output)} \\ \hline \hline
    Ontologies & & \\  \hline \hline
    Concepts & & \\  \hline
    Concept merges & n/a &  \\ \hline 
    Mappings & &  \\  \hline \hline
    Connected subgraphs & & 1  \\ \hline
    Hierarchy edges & & \\   \hline
    Parent concepts & & \\  \hline
    Leaf concepts & &  \\ \hline
    Sibling concepts (min, mean, max) & &  \\ \hline
\end{tabular}
}
\caption{Input and output (domain ontology) comparison}
\end{table}

==> tables/node_status.tex <==
\begin{table}[!ht]
% \label{eval:node_status_deduplication_and_connectivity}
\centering
\scalebox{0.80}{
\begin{tabular}{|l|l|r|r|}
\hline
    \textbf{Stage} & \textbf{Concept set} & \textbf{Count} & \textbf{Ratio (\%)} \\ \hline \hline
    \multirow{5}{*}{Deduplication} & \textit{Input} & 115,934 & 100.00\% \\ \cline{2-4}
     & (Mapped by default) Seed & 21,912 & 18.90\% \\ \cline{2-4}
     & Mapped to Seed & 22,407 & 19.33\% \\ \cline{2-4}
     & Mapped to other (excluding to seed) & 0 & 0.0\% \\ \cline{2-4}
     & \textit{Unmapped} & 71,615 & 61.77\% \\ \hline \hline
    \multirow{5}{*}{Connectivity} & \textit{Input} & 93,527 & 100.00\% \\ \cline{2-4}
     & (Connected by default) Seed & 21,912 & 23.42\% \\ \cline{2-4}
     & Connected to Seed & 0 & 0.0\% \\ \cline{2-4}
     & Connected to other than seed & 705 & 0.75\% \\ \cline{2-4}
     & \textit{Disconnected} & 70,640 & 75.83 \% \\ \hline
\end{tabular}
}
\caption{Concept deduplication and connectivity status}
\end{table}
